Prototypical Fine-tuning: Towards Robust Performance Under Varying Data Sizes

In this paper, we move towards combining large parametric models with non-parametric prototypical networks. We propose prototypical fine-tuning, a novel prototypical framework for fine-tuning pretrained language models (LM), which automatically learns a bias to improve predictive performance for varying data sizes, especially low-resource settings. Our prototypical fine-tuning approach can automatically adjust the model capacity according to the number of data points and the model's inherent attributes. Moreover, we propose four principles for effective prototype fine-tuning towards the optimal solution. Experimental results across various datasets show that our work achieves significant performance improvements under various low-resource settings, as well as comparable and usually better performances in high-resource scenarios.

==> impact.tex <==
\section{Broader Impact}

Many language models exhibit socially problematic biases derived from the pretraining corpora~\cite{bordia2019identifying}. Due to the mechanism of prototypical networks, although our method may reflect these biases through prototype embeddings and predictions, it can also serve to pinpoint, explain, and correct these biases.

% Recent literature have highlighted the significance of forecasting ML model performances when they are initially developed~\cite{nair2021changed}. 

% In this sense, the model after \emph{random subset initialization} may 
% The initially generated prototypes may provide the additional benefit of comparing pretrained models performances at a low cost before training starts~\cite{nair2021changed}. We believe that prototypes can serve as a tool for model selection and explaining model differences.
% This result has a substantial practical usage when fine-tuning is costly and opens up a potential research direction about the correlations between transformer models' pretrained representations and their final performances.
